CONCORD: Towards a DSL for Configurable Graph Code Representation

Deep learning is widely used to uncover hidden patterns in large code corpora. To achieve this, constructing a format that captures the relevant characteristics and features of source code is essential. Graph-based representations have gained attention for their ability to model structural and semantic information. However, existing tools lack flexibility in constructing graphs across different programming languages, limiting their use. Additionally, the output of these tools often lacks interoperability and results in excessively large graphs, making graph-based neural networks training slower and less scalable. We introduce CONCORD, a domain-specific language to build customizable graph representations. It implements reduction heuristics to reduce graphs' size complexity. We demonstrate its effectiveness in code smell detection as an illustrative use case and show that: first, CONCORD can produce code representations automatically per the specified configuration, and second, our heuristics can achieve comparable performance with significantly reduced size. CONCORD will help researchers a) create and experiment with customizable graph-based code representations for different software engineering tasks involving DL, b) reduce the engineering work to generate graph representations, c) address the issue of scalability in GNN models, and d) enhance the reproducibility of experiments in research through a standardized approach to code representation and analysis.

==> assets/listings/concord_grammar.tex <==
\begin{listing}
\begin{minted}[
fontsize=\footnotesize,
breaklines=true,
samepage=true,
]{python}
Main:
    'Tasks' '{'
        tasks*=Task
    '}'
    'Representations' '{'
        representations+= Representation
    '}';
Representation:
    name=ID '{'
        repo_dirs = STRING
        output_dir = STRING
        base_graph_types+= BaseGraphType
        tasks+=[Task]
    '}';
BaseGraphType:
    'AST'|'CFG'|'PDG';
TasksBlock:
    'tasks' '{'
        tasks*=Task
    '}'
    ;
Task:
    name=ID '{'
        operations+= Operation
        'conditions' '{'
        conditions+=Condition
        '}'
    '}'
;
Operation:
    graph_element=GraphElement operation_type=OperationType graph_element_type=GraphElementType
;
GraphElement:
    'Node'|'Edge'
;
OperationType:
    'add'|'remove'
;
GraphElementType:
    EdgeType|NodeType
;
EdgeType:
    'next_token'|'next_sibling'|'for_cfg'|'while_cfg'|'last_read_write'|'guarded_by'|'returns_to'|'computed_from'|'last_lexical_use'
;
NodeType:
    'print'|'logging'|'sys_exit'|'simple_assignment'
;
Condition:
    CodeCondition|StructuralCondition
;
CodeCondition:
    action=CodeConditionAction code_block=CodeBlock
;
CodeConditionAction:
    'exclude'|'include'
;
StructuralCondition:
    graph_element=GraphElement property=StructuralConditionProperty spec=StructuralConditionSpec
    ;
StructuralConditionProperty:
    'count'
    ;
StructuralConditionSpec:
    '['lbound=NUMBER ','ubound=NUMBER ']'
    ;
CodeBlock:
    'catch'|'for'|'while'|'if'|'else'
    ;
Comment:
  /\/\*(.|\n)*?\*\// | /\/\/.*?$/
  ;
\end{minted}
\caption{\concord{}'s textx grammar.}
\label{lst:concord_grammar}
\end{listing}

==> assets/listings/r1.tex <==
\begin{lstlisting}[
   style=concord_style,
    basicstyle=\tiny,
   caption={{\rone} Representation},
   language=HTML,
   label={lst:r1},
]
Tasks {
    task1 {
        Edge add next_token
        Edge add for_cfg
        Edge add while_cfg
        Edge add computed_from
        Edge add guarded_by
        conditions {
            exclude while_block
            exclude if_block
}}}
Representations {
    r1 {
        "/dir/repos_list.csv"
        "output_dir"
        AST
        task1
}}
\end{lstlisting}

==> assets/listings/r3.tex <==
\begin{lstlisting}[
   style=concord_style,
    basicstyle=\tiny,
   caption={{\rthree} Representation},
   language=HTML,
   label={lst:r3},
]
Tasks {
    task3 {
        Edge add next_token
        Edge add for_cfg
        Edge add while_cfg
        Edge add computed_from
        Edge add guarded_by
        Node remove print
        conditions {
            exclude while_block
            exclude if_block
}}}
Representation {
    r3 {
        "/dir/repos_list.csv"
        "output_dir"
        AST
        task3
}}
\end{lstlisting}

==> assets/listings/temp_vars_python.tex <==
\begin{lstlisting}[
    style=python,
    basicstyle=\small,
    caption={Example of a Python code snippet with temporary variables},
   label={lst:example_temp_py},
]
def sum_even_numbers(numbers):
    result = 0
    for number in numbers:
        if number % 2 == 0:
            result += number
    print("The sum of even numbers is:", result)
    return result

\end{lstlisting}

==> assets/tables/classification_results_baseline.tex <==
\begin{table*}
  \centering
  \caption{Classification Results of the Baseline Models}
    \begin{tabular}{@{} l *{4}{ccccc} @{}}
    \toprule
          & \multicolumn{4}{c}{CM} & \multicolumn{4}{c}{CC} & \multicolumn{4}{c}{FE} & \multicolumn{4}{c}{MFA} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
          & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{MCC} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{MCC} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{MCC} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{MCC} \\
    \midrule
    AutoEncoder 1D &0.2& 0.0008& 0.001& 0.009  & 0.41 & 0.002 & 0.004 & 0.023 &  &  &  &  &  &  &  &  &  \\
    ConvNN 1D &  0.67 & 0.36 & 0.47 & 0.45 & 0.59 & 0.24 & 0.34 & 0.36 & 0.57 & 0.05 & 0.09 & 0.17 & - & - & - & -  \\
    ConvNN 2D &  0.61 & 0.62 & 0.62 & 0.59 & 0.55 & 0.55 & 0.55 & 0.53 & - & - & - & - &  - & - & - & -   \\
    RecurrentNN 1D  & 0.93 & 0.33 & 0.48 & 0.53 & 0.66 & 0.001 & 0.003 & 0.032  &  &  &  &  &  &  &  \\
    \bottomrule
    \end{tabular}%
  \label{tab:baseline_results}%
\end{table*}%

==> assets/tables/performance_r2_r3_on_r1.tex <==
\begin{table*}
\centering
\caption{Performance of models trained on {\rtwo} and {\rthree} evaluated on {\rone} data.}
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{4}{c}{R2} & \multicolumn{4}{c}{R3} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
 & P & R & F1 & MCC & P & R & F1 & MCC  \\
\midrule
Complex Method & 0.50 & 0.46 & 0.45 & 0.45 & 0.51 & 0.48 & 0.46 & 0.46 \\
Complex Conditional & 0.48 & 0.43 & 0.44 & 0.44 & 0.43 & 0.40 & 0.40 & 0.40\\
Feature Envy & 0.53 & 0.63 & 0.55 & 0.47 & 0.51 & 0.67 & 0.53 & 0.46\\
Multifaceted Abstraction & 0.52 & 0.16 & 0.24 & 0.25 & 0.52 & 0.13 & 0.21 & 0.21 \\
\bottomrule
\end{tabular}
\label{tab:classification_results_r2_r3_on_r3}
\end{table*}

==> sections/5-related-work.tex <==
In this section, we provide a discussion of the related works that pertain to \dsl{}s in software engineering, the tools and techniques used for constructing program graphs under different representations and studies that address the problem of program reduction.
\subsection{Domain Specific Languages in Sofware Engineering}
There have been many \dsl{} proposed in software engineering literature \cite{Thanhofer2017}.
For example,
Pig Latin \cite{Olston2008PigLA} is a textual \dsl{} that abstracts the MapReduce implementation. 
The \dsl{} code is translated by the compiler into MapReduce jobs that are executed by the infrastructure provided by Apache Hadoop. 
% It also offers extra features such as assistance in the parallel execution of algorithms and matrix and vector arithmetic. 
Andrzejak \etal{} proposed {\sc nldsl} \cite{Andrzejak2019} that is used to create chain and pipeline operations for data processing. 
% Instructions defined by users for data manipulation are transformed into Python code depending on the specified data analysis framework (Pandas or PySpark).
{\sc scope} \cite{SCOPE2008} was developed by Microsoft to help parallel manipulation of large data. Our work differs because we are addressing a different kind of concern from those stated here.
\subsection{Tools for Constructing Graphs}
Bieber et al. \cite{Bieber2022} provides an open-source Python library called \textit{python\_graphs} 
to construct graph representations of Python programs by employing static analysis, 
thereby making it suitable for training machine learning models. 
The library is capable of constructing control-flow graphs, data-flow graphs, and composite ``program graphs'' that combine control-flow, data-flow, syntactic, and lexical information about a program. 
Furthermore, the authors have incorporated a subset of edge augmentation
% which was gathered from the literature, that is 
similar to \concord{}. 
% The authors emphasize the capabilities and limitations of the library and showcase its usefulness for machine learning research by performing a case study, where the library was applied to millions of competitive programming submissions. 
Rice \etal{} \cite{Rice2018} developed a \textit{javac} plugin \textit{feature-javac} that constructs feature graphs for Java-based source code repositories. 
These graphs incorporate a variety of syntactic and semantic features. 
It bears similarities with the \textit{python\_graphs} library and has been designed to facilitate machine learning on source code research.

There are two distinct differences between \concord{} and the above-mentioned tools. 
Firstly, each tool exclusively supports a particular programming language, either Python or Java, thereby limiting their applicability to those languages only. 
In contrast, \concord{} utilizes \textit{joern} in its backend, enabling it to support multiple programming languages such as Java, C, C++, Kotlin, PHP, Python, and JavaScript. 
Additionally, it provides a feature for graph size reduction, which reduces the computational costs of training graph neural networks.
%\todo{configurability is another big difference}
In addition, a significant advantage of \concord{} lies in its capability for composability and configurability of diverse modelling techniques. For example, if a user intends to introduce the {\sc{WhileCFG}} relation to the representation created by \cite{Rice2018}, they are obliged to modify and re-implement the logic from the beginning. Regarding configurability, the tools developed by \cite{Rice2018} and \cite{Bieber2022} do not offer the flexibility to specify which types of relationships to include. Instead, the resulting structures consist of all implemented relations. To address this issue, \concord{} provides the ability to define multiple representations, each of which can differ to satisfy the modelling objectives of the user.
\subsection{Source Code Reduction}
Zhang \etal{} \cite{Zhang2022} introduce an approach called \textit{DietCode} that leverages large pre-trained models such as CodeBERT for source code. 
Through an empirical analysis of CodeBERT's attention mechanism, 
they discovered that the model focuses more on certain types of tokens and statements such as keywords and data-relevant statements. 
Based on this finding, they proposed three strategies for simplifying CodeBERT's input program: 
word dropout, 
frequency filtering, 
and an attention-based approach that selects statements and tokens with the highest attention weights. 
They tested the efficacy of DietCode on code search and code summarization tasks and found that it performs comparably to CodeBERT while requiring 40\% less computational cost during fine-tuning and testing.
Rabin \etal{} \cite{Rabin2021} propose \textsc{sivand}, 
which employs delta debugging to identify the most critical code segments for a deep learning model. 
This technique involves a deep learning model receiving a code snippet as input, which is subsequently segmented. 
The neural network model then processes each segment for a downstream task, such as method name prediction. 
If a segment achieves a desirable score, it is further divided. 
This iterative process continues until the subset's performance fails to meet the targeted score. 
Ultimately, the algorithm produces the smallest code snippet that satisfies the model's objective.
In contrast to DietCode and \textsc{sivand}, \concord{} does not rely on the use of a deep learning model for program simplification. 
Instead, the reduction process takes place during the graph construction stage, 
without the need for extra computation. 
As a result, it is computationally less demanding. For instance, \textsc{sivand} requires the execution and evaluation of a deep learning model at each stage of program reduction, which can be inefficient if the data scales upwards.
